Lax Modal Lambda Calculi

Intuitionistic modal logics (IMLs) extend intuitionistic propositional logic with modalities such as the box and diamond connectives. Advances in the study of IMLs have inspired several applications in programming languages via the development of corresponding type theories with modalities. Until recently, IMLs with diamonds have been misunderstood as somewhat peculiar and unstable, causing the development of type theories with diamonds to lag behind type theories with boxes. In this article, we develop a family of typed-lambda calculi corresponding to sublogics of a peculiar IML with diamonds known as Lax logic. These calculi provide a modal logical foundation for various strong functors in typed-functional programming. We present possible-world and categorical semantics for these calculi and constructively prove normalization, equational completeness and proof-theoretic inadmissibility results. Our main results have been formalized using the proof assistant Agda.

==> lib/macros.tex <==
\makeatletter
\DeclareRobustCommand{\mycircle}{\mathord{\mathpalette\is@circle\relax}}
\newcommand\is@circle[2]{%
  \begingroup
  \sbox\z@{\raisebox{\depth}{$\m@th#1\bigcirc$}}%
  \sbox\tw@{$#1\square$}%
  \resizebox{!}{\ht\tw@}{\usebox{\z@}}%
  \endgroup
}
\makeatother



%\DeclareSymbolFont{system}{T1}{cmr}{m}{sc}
\makeatletter
\def\system@font{\rmfamily}
\def\systemfont{\system@font}
\NewDocumentCommand{\DeclareSystem}{mmm}{%
  \expandafter\DeclareRobustCommand\expandafter{\csname#1\endcsname}{{\system@font\glsfmttext{#1}}\xspace}
  \expandafter\DeclareRobustCommand\expandafter{\csname#1s\endcsname}{{\system@font\glsentryplural{#1}}\xspace}
  \newglossaryentry{#1}{%
    name={#2},
    description={#3}
  }
}
\makeatother

\makeatletter
\NewDocumentCommand\dependson{mom}{%
  \@ifpackageloaded{#1}{%
    #3
  }{%
    \IfValueTF{#2}{
      \PackageWarningNoLine{macros}{Load package `#1' for #2}
    }{%
      \PackageWarningNoLine{macros}{Package `#1' needed for some macros but missing}
    }
  }
}
\NewDocumentCommand\dependsoncommand{mom}{%
  \ifcsname #1\endcsname
    #3
  \else
    \IfValueTF{#2}{
      \PackageWarningNoLine{macros}{Define command `#1' for #2}
    }{%
      \PackageWarningNoLine{macros}{Command `#1' needed for some macros but missing}
    }
  \fi
}
\makeatother



\NewDocumentCommand{\thyeq}{}{\sim} % axiomatic equality (of an equational theory, in a quotient, any congruence relation)

% type operators
\NewDocumentCommand{\CircTy}{g}{\mycircle\IfValueT{#1}{#1}}
\NewDocumentCommand{\BoxTy}{g}{\square\IfValueT{#1}{#1}}
\NewDocumentCommand{\DiaTy}{g}{\lozenge\IfValueT{#1}{#1}}
\DeclareTypeInfix{\FunTy}{\Rightarrow}
\DeclareTypeInfix{\ProdTy}{\times}
\NewDocumentCommand{\BlackDiaTy}{g}{\blacklozenge\IfValueT{#1}{#1}}

% term operators

\DeclareTermOperator{\lamLabel}{lam}
\NewDocumentCommand{\lamTm}{mm}{\lamLabel\,#1.\,#2}

\DeclareTermOperator{\appTm}{app}
\DeclareTermOperator{\unitTm}{unit}
\DeclareTermOperator{\pairTm}{pair}
\DeclareTermOperator{\fstTm}{fst}
\DeclareTermOperator{\sndTm}{snd}
\DeclareTermOperator{\upTm}{up}

\DeclareTermOperator{\inLabel}{in}

\DeclareTermOperator{\returnLLTm}{return_{\text{\ML}}}
\DeclareTermOperator{\letLLTm}{let_{\text{\ML}}}
\NewDocumentCommand{\letInLLTm}{ggg}{\letLLTm{#1=#2\,\inLabel\,}{#3}}

\DeclareTermOperator{\letSLTm}{letmap_{\text{\SL}}}
\NewDocumentCommand{\letInSLTm}{ggg}{\letSLTm{#1=#2\,\inLabel\,}{#3}}

\DeclareTermOperator{\returnRLTm}{return_{\text{\RL}}}
\DeclareTermOperator{\letRLTm}{letmap_{\text{\RL}}}
\NewDocumentCommand{\letInRLTm}{ggg}{\letRLTm{#1=#2\,\inLabel\,}{#3}}

\DeclareTermOperator{\letMapJLTm}{letmap_{\text{\JL}}}
\DeclareTermOperator{\letJoinJLTm}{let_{\text{\JL}}}
\NewDocumentCommand{\letMapInJLTm}{ggg}{\letMapJLTm{#1=#2\,\inLabel\,}{#3}}
\NewDocumentCommand{\letJoinInJLTm}{ggg}{\letJoinJLTm{#1=#2\,\inLabel\,}{#3}}

% context operators
\DeclareTermConstant{\EmptyCtx}{{\cdot}}
\NewDocumentCommand{\ExtCtx}{mm}{#1, #2}
\NewDocumentCommand{\ProdCtx}{mm}{#1, #2}

% for contexts
\NewDocumentCommand{\Wk}{mm}{#1 \subseteq #2}
\def\cesymb{\vartriangleleft}
% \def\cesymb{\sqsubset}
\NewDocumentCommand{\R}{mm}{#1 \cesymb #2}
\NewDocumentCommand{\RLL}{mm}{#1 \cesymb_{\text{\LL}} #2}
\NewDocumentCommand{\RSL}{mm}{#1 \cesymb_{\text{\SL}} #2}
\NewDocumentCommand{\RRL}{mm}{#1 \cesymb_{\text{\RL}} #2}
\NewDocumentCommand{\RJL}{mm}{#1 \cesymb_{\text{\JL}} #2}
\NewDocumentCommand{\Cov}{mm}{#1 \cesymb^* #2}

% for extensions
\DeclareTermOperator{\nilExt}{nil}
\DeclareTermOperator{\varExt}{cons}
\DeclareTermOperator{\varExtOnce}{single}

% for domains of a typed lambda calculus model
\DeclareMathConstant{\Ctx}{Ctx}
\DeclareMathConstant{\Ty}{Ty} % nondependent types
\DeclareMathConstant{\RawTm}{Tm} 
\NewDocumentCommand{\Tm}{mm}{#1 \vdash #2} % don't \DeclareMathInfix in case the prefix notation Tm(Γ,A) will be preferred
\NewDocumentCommand{\Ne}{mm}{#1 \vdashNe #2} % ditto
\NewDocumentCommand{\Nf}{mm}{#1 \vdashNf #2} % ditto
% \NewDocumentCommand{\Subst}{mm}{#1 \vdashSub #2} % ditto
\DeclareMathConstant{\Type}{Type}
\DeclareMathConstant{\Prop}{Prop}

% systems
\DeclareSystem{CPL}{CPL}{}
\DeclareSystem{IPL}{IPL}{}
\DeclareSystem{IPLNeg}{$\text{IPL}_{\top,\times,\Rightarrow}$}{}
\DeclareSystem{CK}{K}{} % classical K
\DeclareSystem{HKDia}{$\text{HK}_{\DiaTy{}}$}{} %
\DeclareSystem{WK}{WK}{} % Wijesekera's
\DeclareSystem{IK}{IK}{} % Wijesekera's 

\DeclareSystem{SL}{SL}{}
\DeclareSystem{RL}{SRL}{}
\DeclareSystem{JL}{SJL}{}
\DeclareSystem{ML}{ML}{}
\DeclareSystem{LL}{PLL}{}

\DeclareSystem{CL}{CL}{}

\DeclareSystem{STLC}{STLC}{}
\DeclareSystem{SLC}{\protect\textnormal{\textlambda}\textsubscript{\SL}}{}
\DeclareSystem{RLC}{\protect\textnormal{\textlambda}\textsubscript{\RL}}{}
\DeclareSystem{JLC}{\protect\textnormal{\textlambda}\textsubscript{\JL}}{}
%\DeclareSystem{LLC}{\protect\textnormal{\textlambda}\textsubscript{\LL}}{}
\DeclareSystem{MLC}{\protect\textnormal{\textlambda}\textsubscript{\ML}}{}

\NewDocumentCommand{\Ri}{}{\mathrel{R_i}}
\DeclareMathOperator{\reflRi}{refl_{i}}
\DeclareMathOperator{\transRi}{trans_{i}}
\NewDocumentCommand{\Rm}{}{\mathrel{R_m}}
\DeclareMathOperator{\reflRm}{refl_{m}}
\DeclareMathOperator{\transRm}{trans_{m}}
\DeclareMathOperator{\incl}{incl}

\DeclareMathOperator{\NfPsh}{Nf}
\DeclareMathOperator{\NePsh}{Ne}

% axioms
\def\KA    {\TirName{K}\xspace}
\def\SA    {\TirName{S}\xspace}
\def\RA    {\TirName{R}\xspace}
\def\JA    {\TirName{J}\xspace}
\def\TA    {\TirName{T}\xspace}
\def\FourA {\TirName{4}\xspace}

% for derivations
\NewDocumentCommand{\vdashVar}{}{\vdash_{\textsc{var}}}
\NewDocumentCommand{\vdashNf}{}{\vdash_{\textsc{nf}}}
\NewDocumentCommand{\vdashNe}{}{\vdash_{\textsc{ne}}}
\NewDocumentCommand{\vdashSub}{}{\vdash_{\textsc{s}}}

% frames
\NewDocumentCommand{\pr}{}{{\fontfamily{qtm}\selectfont pr}}

\DeclareTypeConstant{\BaseTy}{\iota}
\DeclareTypeConstant{\UnitTy}{1}
\DeclareTypeOperator{\ArrTy}{Array}
\DeclareTypeOperator{\WriterTy}{Writer}
\DeclareTypeOperator{\StateTy}{State}
\DeclareTypeOperator{\MaybeTy}{Maybe}
\DeclareTypeOperator{\ExceptTy}{Except}
\DeclareTypeOperator{\CovTy}{Cov}

\dependson{mathtools}[\string\eval]{%
  \let\evallbracket\llbracket
  \let\evalrbracket\rrbracket
  \DeclarePairedDelimiter\eval\evallbracket\evalrbracket
}

\let\quote=\relax
\DeclareMathOperator{\quote}{quote}
\DeclareMathOperator{\reify}{reify}
\DeclareMathOperator{\reflect}{reflect}
\DeclareMathOperator{\reifyR}{reifyAcc}
\DeclareMathOperator{\norm}{norm}
\DeclareMathOperator{\lookup}{lookup}
\DeclareMathOperator{\idEnv}{idEnv}

\DeclareMathOperator{\factor}{factor}

\DeclareMathOperator{\collect}{collect}
\DeclareMathOperator{\register}{register}

\DeclareMathOperator{\collectSL}{collect_\text{SL}}
\DeclareMathOperator{\registerSL}{register_\text{SL}}

\DeclareMathOperator{\collectRL}{collect_\text{RL}}
\DeclareMathOperator{\registerRL}{register_\text{RL}}

\DeclareMathOperator{\collectJL}{collect_\text{JF}}
\DeclareMathOperator{\registerJL}{register_\text{JF}}

\DeclareMathOperator{\collectLL}{collect_\text{LL}}
\DeclareMathOperator{\registerLL}{register_\text{LL}}

% for weakenings
\DeclareMathConstant{\baseWk}{base}
\DeclareMathOperator{\dropWk}{drop}
\DeclareMathOperator{\keepVarWk}{keep}
\DeclareMathOperator{\keepLockWk}{keep_{\lockCtx}}
\NewDocumentCommand{\subst}{mm}{#1 [#2]}
\DeclareMathOperator{\wkTm}{\uparrow}

\DeclareMathOperator{\monLabel}{mon}
\NewDocumentCommand{\wkPsh}{mmm}{\monLabel_{#1} \, #2\, #3}

\DeclareMathConstant{\idWk}{refl_{\Wk{}{}}}
\DeclareMathOperator{\transWk}{trans_{\Wk{}{}}}
\DeclareMathConstant{\dropIdWk}{new}

% Categorical stuff


\NewDocumentCommand{\CircFun}{g}{\mycircle\IfValueT{#1}{#1}}
\NewDocumentCommand{\CircMap}{g}{\mycircle\IfValueT{#1}{#1}}

\NewDocumentCommand{\DiaFun}{g}{\lozenge\IfValueT{#1}{#1}}
\NewDocumentCommand{\DiaMap}{g}{\lozenge\IfValueT{#1}{#1}}
\DeclareTypeInfix{\FunFun}{\Rightarrow}
\DeclareTypeInfix{\ProdFun}{\times}

\DeclareTypeInfix{\Prod}{\times}

\NewDocumentCommand{\FFun}{g}{F\IfValueT{#1}{#1}}
\NewDocumentCommand{\FMap}{g}{F\IfValueT{#1}{#1}}

\NewDocumentCommand{\Fork}{gg}{\langle{#1},{#2}\rangle}

% for metavariables ranging over presheaves we use \mathcal
\NewDocumentCommand{\mcA}{}{\mathcal{A}}
\NewDocumentCommand{\mcB}{}{\mathcal{B}}

% for metavariables ranging over (categorical) models we use \mathcal
\NewDocumentCommand{\mcC}{}{\mathcal{C}}
\NewDocumentCommand{\mcM}{}{\mathcal{M}}
\NewDocumentCommand{\mcN}{}{\mathcal{N}}



\DeclareMathOperator{\Cover}{Cover}

% logical relations
\DeclareMathOperator{\LR}{L}

